A Matheuristic Approach for Solving a Simultaneous Lot Sizing and Scheduling Problem with Client Prioritization in Tire Industry

This paper introduces an integrated lot sizing and scheduling problem inspired from a real-world application in off-the-road tire industry. This problem considers the assignment of different items on parallel machines with complex eligibility constraints within a finite planning horizon. It also considers a large panel of specific constraints such as: backordering, a limited number of setups, upstream resources saturation and customers prioritization. A novel mixed integer formulation is proposed with the objective of optimizing different normalized criteria related to the inventory and service level performance. Based on this mathematical formulation, a problem-based matheuristic method that solves the lot sizing and assignment problems separately is proposed to solve the industrial case. A computational study and sensitivity analysis are carried out based on real-world data with up to 170 products, 70 unrelated parallel machines and 42 periods. The obtained results show the effectiveness of the proposed approach on improving the company's solution. Indeed, the two most important KPIs for the management have been optimized of respectively 32% for the backorders and 13% for the overstock. Moreover, the computational time have been reduced significantly.

==> biblio.tex <==
@article{Harris,
    author  = {Harris, Ford W.},
    title   = {How many parts to make at once},
    year    = {1913},
    journal = {Factory, The magazine of management},
    volume  = {10},
    number  = {2},
    pages   = {135-152},
}
@article{WW,
    author  = "Wagner, Harvey M. and Whitin, Thomson M. ",
    title   = "Dynamic version of the Economic Lot Size Model",
    year    = "1958",
    journal = "Management Science",
    volume  = "5",
    number  = "1",
    pages   = "89--96"
}
@article{Manne,
    author  = "Manne, Alan S.",
    title   = "How many parts to make at once",
    year    = "1958",
    journal = "Management Science",
    volume  = "4",
    number  = "2",
    pages   = "115--201"
}
@article{bitran1982computational,
  title={Computational complexity of the capacitated lot size problem},
  author={Bitran, Gabriel R and Yanasse, Horacio H},
  journal={Management Science},
  volume={28},
  number={10},
  pages={1174--1186},
  year={1982},
  publisher={INFORMS}
}

@book{brahimi2017production,
  title={Production planning: New lot-sizing models and algorithms},
  author={Brahimi, Nadjib and Dauz{\`e}re-P{\'e}res, St{\'e}phane},
  year={2017},
  publisher={{\'E}ditions universitaires europ{\'e}ennes}
}

@article{drexl1997lot,
	title="Lot sizing and scheduling survey and extensions",
	author="Drexl, Andreas and Kimms, Alf",
	journal="European Journal of Operational Research",
	volume="99",
	number="2",
	pages="221--235",
	year="1997",
	publisher="Elsevier"
}
@article{gicquel2008capacitated,
	title={Capacitated lot sizing models: a literature review},
	author={Gicquel, C{\'e}line and Minoux, Michel and Dallery, Yves},
	year={2008}
}
@book{pinedo2005planning,
  title={Planning and scheduling in manufacturing and services},
  author={Pinedo, Michael L},
  year={2005},
  publisher={Springer}
}


@article{Bahl,
	author  = "Bahl, Harish C. and Ritzman, Larry P. and Gupta, Jatinder N. D.",
	title   = "OR Practice determining Lot Sizes and Resource Requirements: A Review",
	year    = "1987",
	journal = "Operations research",
	volume  = "35",
	number  = "3",
	pages   = "329-345"
}
@article{Karimi,
	author  = "Karimi, B. and Fatemi Ghomi, S. M. T. and Wilson, J. M.",
	title   = "The capacitated lot sizing problem: a review of models and algorithms",
	year    = "2003",
	journal = "Omega",
	volume  = "31",
	number  = "5",
	pages   = "365-378"
}
@book{pochet2006production,
	title="Production planning by mixed integer programming",
	author="Pochet, Yves and Wolsey, Laurence A",
	year="2006",
	publisher="Springer Science \& Business Media"
}
@article{jans2008modeling,
	title={Modeling industrial lot sizing problems: a review},
	author={Jans, Raf and Degraeve, Zeger},
	journal={International Journal of Production Research},
	volume={46},
	number={6},
	pages={1619--1643},
	year={2008},
	publisher={Taylor \& Francis}
}
@article{buschkuhl2010dynamic,
	title={Dynamic capacitated lot-sizing problems: a classification and review of solution approaches},
	author={Buschk{\"u}hl, Lisbeth and Sahling, Florian and Helber, Stefan and Tempelmeier, Horst},
	journal={Or Spectrum},
	volume={32},
	number={2},
	pages={231--261},
	year={2010},
	publisher={Springer}
}
@article{diaz2014review,
	title={A review of discrete-time optimization models for tactical production planning},
	author={D{\'\i}az-Madro{\~n}ero, Manuel and Mula, Josefa and Peidro, David},
	journal={International Journal of Production Research},
	volume={52},
	number={17},
	pages={5171--5205},
	year={2014},
	publisher={Taylor \& Francis}
}
@article{brahimi2017single,
	title={Single-item dynamic lot-sizing problems: An updated survey},
	author={Brahimi, Nadjib and Absi, Nabil and Dauz{\`e}re-P{\'e}r{\`e}s, St{\'e}phane and Nordli, Atle},
	journal={European Journal of Operational Research},
	volume={263},
	number={3},
	pages={838--863},
	year={2017},
	publisher={Elsevier}
}
@article{bahl2009empirical,
	title={An empirical comparison of lot-sizing methods available in an ERP System},
	author={Bahl, Harish C and Bahl, Neelam},
	journal={California Journal of Operations Management},
	volume={7},
	number={1},
	pages={77--83},
	year={2009}
}
@article{akbalik2012polynomial,
	title={Polynomial time algorithms for the constant capacitated single-item lot sizing problem with stepwise production cost},
	author={Akbalik, Ayse and Rapine, Christophe},
	journal={Operations Research Letters},
	volume={40},
	number={5},
	pages={390--397},
	year={2012},
	publisher={Elsevier}
}
@article{onal2016two,
	title={The two-level economic lot sizing problem with perishable items},
	author={{\"O}nal, Mehmet},
	journal={Operations Research Letters},
	volume={44},
	number={3},
	pages={403--408},
	year={2016},
	publisher={Elsevier}
}
@article{billington1986heuristics,
	title={Heuristics for multilevel lot-sizing with a bottleneck},
	author={Billington, Peter J and McClain, John O and Thomas, L Joseph},
	journal={Management Science},
	volume={32},
	number={8},
	pages={989--1006},
	year={1986},
	publisher={INFORMS}
}
@article{tempelmeier1996lagrangean,
	title={A Lagrangean-based heuristic for dynamic multilevel multiitem constrained lotsizing with setup times},
	author={Tempelmeier, Horst and Derstroff, Matthias},
	journal={Management Science},
	volume={42},
	number={5},
	pages={738--757},
	year={1996},
	publisher={INFORMS}
}
@article{maes1986simple,
	title={A simple heuristic for the multi item single level capacitated lotsizing problem},
	author={Maes, Johan and Van Wassenhove, Luk N},
	journal={Operations Research Letters},
	volume={4},
	number={6},
	pages={265--273},
	year={1986},
	publisher={Elsevier}
}
@article{maes1991multilevel,
	title={Multilevel capacitated lotsizing complexity and LP-based heuristics},
	author={Maes, Johan and McClain, John O and Van Wassenhove, Luk N},
	journal={European Journal of Operational Research},
	volume={53},
	number={2},
	pages={131--148},
	year={1991},
	publisher={Elsevier}
}
@article{helber2010fix,
	title={A fix-and-optimize approach for the multi-level capacitated lot sizing problem},
	author={Helber, Stefan and Sahling, Florian},
	journal={International Journal of Production Economics},
	volume={123},
	number={2},
	pages={247--256},
	year={2010},
	publisher={Elsevier}
}
@article{toledo2015relax,
	title={A relax-and-fix with fix-and-optimize heuristic applied to multi-level lot-sizing problems},
	author={Toledo, Claudio Fabiano Motta and da Silva Arantes, M{\'a}rcio and Hossomi, Marcelo Yukio Bressan and Fran{\c{c}}a, Paulo Morelato and Akartunal{\i}, Kerem},
	journal={Journal of Heuristics},
	volume={21},
	number={5},
	pages={687--717},
	year={2015},
	publisher={Springer}
}
@article{behnamian2017markovian,
	title={A Markovian approach for multi-level multi-product multi-period capacitated lot-sizing problem with uncertainty in levels},
	author={Behnamian, J and Fatemi Ghomi, SMT and Karimi, B and Fadaei Moludi, M},
	journal={International Journal of Production Research},
	volume={55},
	number={18},
	pages={5330--5340},
	year={2017},
	publisher={Taylor \& Francis}
}

@article{karimi2003capacitated,
	title={The capacitated lot sizing problem: a review of models and algorithms},
	author={Karimi, Behrooz and Ghomi, SMT Fatemi and Wilson, JM},
	journal={Omega},
	volume={31},
	number={5},
	pages={365--378},
	year={2003},
	publisher={Elsevier}
}
@techreport{miller2000solving,
	title={Solving multi-item capacitated lot-sizing problems with setup times by branch-and-cut},
	author={Miller, Andrew J and Nemhauser, George L and Savelsbergh, Martin WP and others},
	year={2000},
	institution={Universit{\'e} Catholique de Louvain. Center for Operations Research and~…}
}
@article{ceschia2017solving,
	title={Solving discrete lot-sizing and scheduling by simulated annealing and mixed integer programming},
	author={Ceschia, Sara and Di Gaspero, Luca and Schaerf, Andrea},
	journal={Computers \& Industrial Engineering},
	volume={114},
	pages={235--243},
	year={2017},
	publisher={Elsevier}
}
@article{nobil2016single,
	title={A single machine EPQ inventory model for a multi-product imperfect production system with rework process and auction},
	author={Nobil, Amir Hossein and Taleizadeh, Ata Allah},
	journal={International Journal of Advanced Logistics},
	volume={5},
	number={3-4},
	pages={141--152},
	year={2016},
	publisher={Taylor \& Francis}
}
@article{de2007joint,
	title={Joint rolling-horizon scheduling of materials processing and lot-sizing with sequence-dependent setups},
	author={de Araujo, Silvio A and Arenales, Marcos N and Clark, Alistair R},
	journal={Journal of Heuristics},
	volume={13},
	number={4},
	pages={337--358},
	year={2007},
	publisher={Springer}
}
@article{absi2007mip,
	title={MIP-based heuristics for multi-item capacitated lot-sizing problem with setup times and shortage costs},
	author={Absi, Nabil and Kedad-Sidhoum, Safia},
	journal={RAIRO-Operations Research},
	volume={41},
	number={2},
	pages={171--192},
	year={2007},
	publisher={EDP Sciences}
}
@article{gruson2018impact,
  title={The impact of service level constraints in deterministic lot sizing with backlogging},
  author={Gruson, Matthieu and Cordeau, Jean-Fran{\c{c}}ois and Jans, Raf},
  journal={Omega},
  volume={79},
  pages={91--103},
  year={2018},
  publisher={Elsevier}
}
@article{Cattryse,
    author  = "Cattryse, Dirk and Salomon, Marc and Kuik, Roelof and Van Wassenhove, Luk N.",
    title   = "A dual ascent and column generation heuristic for the discrete lotsizing and scheduling problem with setup times",
    year    = "1993",
    journal = "Management Science",
    volume  = "39",
    number  = "4",
 pages   = "477--486"
}
@article{Fleischmann,
    author  = "Fleischmann, Bernhard",
    title   = "The discrete lot sizing and scheduling problem",
    year    = "1990",
    journal = "European journal of operational research",
    volume  = "44",
 pages   = "337--348"
}
@article{Lasdon,
    author  = "Lasdon, L. S. and Terjung, R. C.",
    title   = "An efficient algorithm for multi-item scheduling",
    year    = "1970",
    journal = "Operations Research",
    volume  = "19",
    number  = "4",
 pages   = "946--969",
}
@article{DW,
    author  = "Dantzig, George B. and Wolfe, Philip",
    title   = "Decomposition Principle for Linear Programs",
    year    = "1960",
    journal = "Operations Research",
    volume  = "8",
    number  = "1",
 pages   = "101--111"
}
@article{Degraeve,
    author  = "Degraeve, Zeger and Schrage, Linus",
    title   = "A tire production scheduling system for Bridgestone / Firestone off-the-road",
    year    = "1997",
    journal = "Operations Research",
    volume  = "45",
    number  = "6",
 pages   = "789--796"
}
@article{jans2004industrial,
	title={An industrial extension of the discrete lot-sizing and scheduling problem},
	author={Jans, Raf and Degraeve, Zeger},
	journal={IIE transactions},
	volume={36},
	number={1},
	pages={47--58},
	year={2004},
	publisher={Taylor \& Francis}
}
@article{belvaux2000bc,
	title={bc—prod: A specialized branch-and-cut system for lot-sizing problems},
	author={Belvaux, Gaetan and Wolsey, Laurence A},
	journal={Management Science},
	volume={46},
	number={5},
	pages={724--738},
	year={2000},
	publisher={INFORMS}
}
@article{Dzielinski,
    author  = "Dzielinski, Berard P. and Gomory, Ralph E.",
    title   = "Optimal programming of lot sizes, inventory and labor allocations",
    year    = "1965",
    journal = "Management Science",
    volume  = "11",
    number  = "9",
 pages   = "874--890"
}
@article{nobil2019imperfect,
	title={An imperfect multi-item single machine production system with shortage, rework, and scrapped considering inspection, dissimilar deficiency levels, and non-zero setup times},
	author={Nobil, Amir Hossein and Afshar Sedigh, Amir Hosein and Tiwari, Sunil and Wee, Hui Ming},
	journal={Scientia Iranica},
	volume={26},
	number={1},
	pages={557--570},
	year={2019},
	publisher={Sharif University of Technology}
}
@article{nobil2019imperfect,
	title={An imperfect multi-item single machine production system with shortage, rework, and scrapped considering inspection, dissimilar deficiency levels, and non-zero setup times},
	author={Nobil, Amir Hossein and Afshar Sedigh, Amir Hosein and Tiwari, Sunil and Wee, Hui Ming},
	journal={Scientia Iranica},
	volume={26},
	number={1},
	pages={557--570},
	year={2019},
	publisher={Sharif University of Technology}
}

@article{absi2019worst,
  title={Worst case analysis of Relax and Fix heuristics for lot-sizing problems},
  author={Absi, Nabil and van den Heuvel, Wilco},
  journal={European Journal of Operational Research},
  volume={279},
  number={2},
  pages={449--458},
  year={2019},
  publisher={Elsevier}
}

@article{helber2013dynamic,
	title={Dynamic capacitated lot sizing with random demand and dynamic safety stocks},
	author={Helber, Stefan and Sahling, Florian and Schimmelpfeng, Katja},
	journal={OR Spectrum},
	volume={35},
	number={1},
	pages={75--105},
	year={2013},
	publisher={Springer}
}
@article{ghirardi2019matheuristics,
  title={Matheuristics for the lot sizing problem with back-ordering, setup carry-overs, and non-identical machines},
  author={Ghirardi, Marco and Amerio, Andrea},
  journal={Computers \& Industrial Engineering},
  volume={127},
  pages={822--831},
  year={2019},
  publisher={Elsevier}
}

@article{yalaoui2013fuzzy,
  title={Fuzzy-metaheuristic methods to solve a hybrid flow shop scheduling problem with pre-assignment},
  author={Yalaoui, Naim and Ouazene, Yassine and Yalaoui, Farouk and Amodeo, Lionel and Mahdi, Halim},
  journal={International Journal of Production Research},
  volume={51},
  number={12},
  pages={3609--3624},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{masmoudi2016multi,
  title={Multi-item capacitated lot-sizing problem in a flow-shop system with energy consideration},
  author={Masmoudi, Oussama and Yalaoui, Alice and Ouazene, Yassine and Chehade, Hicham},
  journal={IFAC-PapersOnLine},
  volume={49},
  number={12},
  pages={301--306},
  year={2016},
  publisher={Elsevier}
}
 @misc{michelin_2020,
 title={an unknown object the tire materials},
 author={Michelin},
 year={2020},
 url={https://thetiredigest.michelin.com/an-unknown-object-the-tire-materials} } 
 
  @book{boudha_kumar_srimannarayana_koyan_2011,
  author={Boudha, Arvind and Kumar, Sateesh and Srimannarayana and Koyan, Febin},
  title={Tyre Manufacturing Processes Seminar Report},
  institution={Indian Institute of Technology},
  place={Bombay},
  year={2011}} 
  
  @article{baldo2017alternative,
  title={Alternative mathematical models and solution approaches for lot-sizing and scheduling problems in the brewery industry: Analyzing two different situations},
  author={Baldo, Tamara A and Morabito, Reinaldo and Santos, Maristela O and Guimar{\~a}es, Luis},
  journal={Mathematical Problems in Engineering},
  volume={2017},
  pages={1--18},
  year={2017},
  publisher={Hindawi}
}

@article{chen2015fix,
  title={Fix-and-optimize and variable neighborhood search approaches for multi-level capacitated lot sizing problems},
  author={Chen, Haoxun},
  journal={Omega},
  volume={56},
  pages={25--36},
  year={2015},
  publisher={Elsevier}
}

@article{copil2017simultaneous,
  title={Simultaneous lotsizing and scheduling problems: a classification and review of models},
  author={Copil, Karina and W{\"o}rbelauer, Martin and Meyr, Herbert and Tempelmeier, Horst},
  journal={OR Spectrum},
  volume={39},
  number={1},
  pages={1--64},
  year={2017},
  publisher={Springer}
}
  
 @article{cunha2018integrated,
  title={An integrated approach for production lot sizing and raw material purchasing},
  author={Cunha, Artur Lovato and Santos, Maristela Oliveira and Morabito, Reinaldo and Barbosa-P{\'o}voa, Ana},
  journal={European Journal of Operational Research},
  volume={269},
  number={3},
  pages={923--938},
  year={2018},
  publisher={Elsevier}
}

@article{goren2015solving,
  title={Solving the capacitated lot sizing problem with setup carryover using a new sequential hybrid approach},
  author={G{\"o}ren, Hacer G{\"u}ner and Tunal{\i}, Semra},
  journal={Applied Intelligence},
  volume={42},
  number={4},
  pages={805--816},
  year={2015},
  publisher={Springer}
}

@article{li2017fix,
  title={Fix-and-optimize and variable neighborhood search approaches for stochastic multi-item capacitated lot-sizing problems},
  author={Li, Liuxi and Song, Shiji and Wu, Cheng and Wang, Rui},
  journal={Mathematical Problems in Engineering},
  volume={2017},
  number={2},
  year={2017},
  publisher={Hindawi}
}

@article{toledo2016mathematical,
  title={Mathematical programming-based approaches for multi-facility glass container production planning},
  author={Toledo, Claudio Fabiano Motta and da Silva Arantes, Marcio and Hossomi, Marcelo Yukio Bressan and Almada-Lobo, Bernardo},
  journal={Computers \& Operations Research},
  volume={74},
  pages={92--107},
  year={2016},
  publisher={Elsevier}
}

@article{toledo2015synchronized,
  title={The synchronized and integrated two-level lot sizing and scheduling problem: evaluating the generalized mathematical model},
  author={Toledo, Claudio FM and Kimms, Alf and Fran{\c{c}}a, Paulo M and Morabito, Reinaldo},
  journal={Mathematical Problems in Engineering},
  volume={2015},
  pages={1--18},
  year={2015},
  publisher={Hindawi}
}

@Article{Worbelauer2019Simultaneous,
    title={{Simultaneous lotsizing and scheduling considering secondary resources: a general model, literature review and classification}},
    author={Martin Wörbelauer and Herbert Meyr and Bernardo Almada-Lobo},
  journal={OR Spectrum},
  year= {2019},
  volume={41},
  number={1},
  pages={1-43},

}

@article{de2008lot,
  title={Lot sizing and furnace scheduling in small foundries},
  author={de Araujo, Silvio A and Arenales, Marcos N and Clark, Alistair R},
  journal={Computers \& Operations Research},
  volume={35},
  number={3},
  pages={916--932},
  year={2008},
  publisher={Elsevier}
}

@article{deeratanasrikul2017multiple,
  title={Multiple-stage multiple-machine capacitated lot-sizing and scheduling with sequence-dependent setup: A case study in the wheel industry},
  author={Deeratanasrikul, Lalida and Mizuno, Shinji},
  journal={Journal of Industrial \& Management Optimization},
  volume={13},
  number={1},
  pages={413},
  year={2017},
  publisher={American Institute of Mathematical Sciences}
}

@article{gnoni2003production,
  title={Production planning of a multi-site manufacturing system by hybrid modelling: A case study from the automotive industry},
  author={Gnoni, MG and Iavagnilio, R and Mossa, G and Mummolo, G and Di Leva, A},
  journal={International Journal of Production Economics},
  volume={85},
  number={2},
  pages={251--262},
  year={2003},
  publisher={Elsevier}
}

@article{ramezanian2017simultaneous,
  title={A simultaneous planning of production and scheduling operations in flexible flow shops: case study of tile industry},
  author={Ramezanian, Reza and Sanami, Sahar Fallah and Nikabadi, Mohsen Shafiei},
  journal={The International Journal of Advanced Manufacturing Technology},
  volume={88},
  number={9-12},
  pages={2389--2403},
  year={2017},
  publisher={Springer}
}

@article{figueira2013hybrid,
  title={A hybrid VNS approach for the short-term production planning and scheduling: A case study in the pulp and paper industry},
  author={Figueira, Gon{\c{c}}alo and Santos, Maristela Oliveira and Almada-Lobo, Bernardo},
  journal={Computers \& Operations Research},
  volume={40},
  number={7},
  pages={1804--1818},
  year={2013},
  publisher={Elsevier}
}

@article{lasdon1971efficient,
  title={An efficient algorithm for multi-item scheduling},
  author={Lasdon, Leon S and Terjung, RC},
  journal={Operations Research},
  volume={19},
  number={4},
  pages={946--969},
  year={1971},
  publisher={INFORMS}
}

@article{degraeve1997tire,
  title={A tire production scheduling system for Bridgestone/Firestone Off-The-Road},
  author={Degraeve, Zeger and Schrage, Linus},
  journal={Operations Research},
  volume={45},
  number={6},
  pages={789--796},
  year={1997},
  publisher={INFORMS}
}

@article{babaei2014genetic,
  title={A genetic algorithm for the simultaneous lot sizing and scheduling problem in capacitated flow shop with complex setups and backlogging},
  author={Babaei, Mohammad and Mohammadi, Mohammad and Ghomi, SMT Fatemi},
  journal={The International Journal of Advanced Manufacturing Technology},
  volume={70},
  number={1-4},
  pages={125--134},
  year={2014},
  publisher={Springer}
}

@article{vincent2020population,
  title={A population-based metaheuristic for the capacitated lot-sizing problem with unrelated parallel machines},
  author={Vincent, Benjamin and Duhamel, Christophe and Ren, Libo and Tchernev, Nikolay},
  journal={International Journal of Production Research},
  volume={58},
  number={21},
  pages={6689--6706},
  year={2020},
  publisher={Taylor \& Francis}
}

@article{meyr2013decomposition,
  title={A decomposition approach for the general lotsizing and scheduling problem for parallel production lines},
  author={Meyr, Herbert and Mann, Matthias},
  journal={European Journal of Operational Research},
  volume={229},
  number={3},
  pages={718--731},
  year={2013},
  publisher={Elsevier}
}

@article{toscano2020formulation,
  title={Formulation and MIP-heuristics for the lot sizing and scheduling problem with temporal cleanings},
  author={Toscano, Alyne and Ferreira, Deisemara and Morabito, Reinaldo},
  journal={Computers \& Chemical Engineering},
  volume={142},
  pages={107038},
  year={2020},
  publisher={Elsevier}
}

@article{mohammadi2011genetic,
  title={A genetic algorithm for simultaneous lotsizing and sequencing of the permutation flow shops with sequence-dependent setups},
  author={Mohammadi, Mohammad and Ghomi, SMT Fatemi and Jafari, Niloofar},
  journal={International Journal of Computer Integrated Manufacturing},
  volume={24},
  number={1},
  pages={87--93},
  year={2011},
  publisher={Taylor \& Francis}
}

@article{ruiz2005solving,
  title={Solving the flowshop scheduling problem with sequence dependent setup times using advanced metaheuristics},
  author={Ruiz, Rub{\'e}n and Maroto, Concepcion and Alcaraz, Javier},
  journal={European Journal of Operational Research},
  volume={165},
  number={1},
  pages={34--54},
  year={2005},
  publisher={Elsevier}
}

@article{koch2020dedicated,
  title={A dedicated lot sizing problem in tire industry},
  author={ Koch, Cyril and Arbaoui, Taha and Ouazene, Yassine and De Wulf, Antoine and Jaunet, Nicolas},
 journal={IFAC World Congress, Berlin, IFAC-PapersOnline},
  year={2020},
  publisher={Elsevier}
}

@article{koch2021Capacitated,
  title={Capacitated Multi-item Lot Sizing Problem with Client Prioritization in Tire Industry},
author={ Koch, Cyril and Ouazene, Yassine and Arbaoui, Taha and Yalaoui, Farouk and De Brunier, Humbert  and Jaunet, Nicolas},
 journal={INCOM21, IFAC-PapersOnLine},
  year={2021},
  publisher={Elsevier}
}

@article{della1995generalized,
  title={Generalized pairwise interchanges and machine scheduling},
  author={Della Croce, Federico},
  journal={European Journal of Operational Research},
  volume={83},
  number={2},
  pages={310--319},
  year={1995},
  publisher={Elsevier}
}
@article{rodoplu2020fix,
  title={A fix-and-relax heuristic for the single-item lot-sizing problem with a flow-shop system and energy constraints},
  author={Rodoplu, Melek and Arbaoui, Taha and Yalaoui, Alice},
  journal={International Journal of Production Research},
  volume={58},
  number={21},
  pages={6532--6552},
  year={2020},
  publisher={Taylor \& Francis}
}

@article{cplex2009v12,
  title={V12. 1: User’s Manual for CPLEX},
  author={Cplex, IBM ILOG},
  journal={International Business Machines Corporation},
  volume={46},
  number={53},
  pages={157},
  year={2009},
  publisher={Armonk, NY, USA}
}

@software{minitab,
  author = {{Minitab, LLC}},
  title = {Minitab},
  url = {https://www.minitab.com},
  version = {20.2},
  date = {2021-04-16},
}

@article{tirkolaee2020fuzzy,
  title={Fuzzy mathematical programming and self-adaptive artificial fish swarm algorithm for just-in-time energy-aware flow shop scheduling problem with outsourcing option},
  author={Tirkolaee, Erfan Babaee and Goli, Alireza and Weber, Gerhard-Wilhelm},
  journal={IEEE transactions on fuzzy systems},
  volume={28},
  number={11},
  pages={2772--2783},
  year={2020},
  publisher={IEEE}
}
